Connecting MapReduce Computations to Realistic Machine Models

We explain how the popular, highly abstract MapReduce model of parallel computation (MRC) can be rooted in reality by explaining how it can be simulated on realistic distributed-memory parallel machine models like BSP. We first refine the model (MRC$^+$) to include parameters for total work $w$, bottleneck work $\hat{w}$, data volume $m$, and maximum object sizes $\hat{m}$. We then show matching upper and lower bounds for executing a MapReduce calculation on the distributed-memory machine -- $\Theta(w/p+\hat{w}+\log p)$ work and $\Theta(m/p+\hat{m}+\log p)$ bottleneck communication volume using $p$ processors.

==> abstract.tex <==
 Tools like MapReduce/Hadoop, Spark or Thrill have ``democratized''
massively parallel computing. What was previously only used for
numerical simulations that need investments of many person-years to
get an application running is now used for a wide range of ``big
data'' applications. Simple applications can be built within an hour
and there is a rather gentle learning curve. One reason for this
success is that a simple operation like the MapReduce transformation
of multisets can express a large range of applications. The tools can
automatically handle difficult issues like parallelization, load
balancing, fault tolerance, and management of the memory hierarchy.

The algorithm theory community has complemented this success by
introducing a complexity model (\MRC) that basically counts the number of
required MapReduce calculations for solving a problem. However, this
has opened a large gap between theory and practice. When does a
particular MapReduce algorithm really allow efficient parallel
execution? Is Algorithm~A really superior to Algorithm~B only because
it needs fewer steps? Many papers therefore discuss additional
characteristics of these algorithms like the volume of generated
intermediate data.

We put such refinements of the MapReduce model (\MRCplus) on a solid basis by
precisely defining the requirements on a MapReduce algorithm to
achieve efficient execution on realistic models of computing.  Not
surprisingly, additional parameters are total work $w$, bottleneck
work $\hat{w}$, data volume $m$, and maximum object sizes $\hat{m}$.
The main contribution of this paper is to prove that, in some sense,
these parameters fully characterize the difficulty of a MapReduce step
by proving matching lower and upper bounds for executing them on a
distributed-memory machine.  We begin with a simple algorithm for the
BSP model based on oblivious random dispersal of work. Then we
introduce an asynchronous distributed-memory work-stealing algorithm
that optimally adapts to imbalance in unpredictable local
computations. Using an adaptive shuffling operation and measures for
balancing the amount of output data, we finally arrive at an optimal
MapReduce algorithm that does $\Oh{w/p+\hat{w}+\log p}$ local work requiring
$\Oh{m/p+\hat{m}+\log p}$ bottleneck communication volume on $p$ processors.

We give
evidence that such algorithms might also help to arrive at more
scalable MapReduce implementations in practice. We formulate open problems with
respect to handling fault-tolerance, the memory hierarchy, and a
richer set of supported operations.

